Reaching the Limit in Autonomous Racing: Optimal Control versus Reinforcement Learning

A central question in robotics is how to design a control system for an agile mobile robot. This paper studies this question systematically, focusing on a challenging setting: autonomous drone racing. We show that a neural network controller trained with reinforcement learning (RL) outperformed optimal control (OC) methods in this setting. We then investigated which fundamental factors have contributed to the success of RL or have limited OC. Our study indicates that the fundamental advantage of RL over OC is not that it optimizes its objective better but that it optimizes a better objective. OC decomposes the problem into planning and control with an explicit intermediate representation, such as a trajectory, that serves as an interface. This decomposition limits the range of behaviors that can be expressed by the controller, leading to inferior control performance when facing unmodeled effects. In contrast, RL can directly optimize a task-level objective and can leverage domain randomization to cope with model uncertainty, allowing the discovery of more robust control responses. Our findings allowed us to push an agile drone to its maximum performance, achieving a peak acceleration greater than 12 times the gravitational acceleration and a peak velocity of 108 kilometers per hour. Our policy achieved superhuman control within minutes of training on a standard workstation. This work presents a milestone in agile robotics and sheds light on the role of RL and OC in robot control.

==> Images/drone_tikz.tex <==
\begin{table}[!htp]
    % \small
    \centering
    \fontsize{9pt}{12pt}\selectfont   
    \caption{The drone used for the real-world experiment. The drone has a maximum thrust-to-weight ratio of 9.74, making it the most aggressive autonomous drone.   }
    \label{tab:physical_drone}
    \begin{tabular}{ m{6.2cm} c | c }
        \toprule
        \multirow{6}{*}{\includegraphics[width=1.0\linewidth]{Images/drone.jpg}}
        % \includegraphics[width=0.4\linewidth]{Images/drone.jpg}
         & \textbf{Parameter} & \textbf{Value}  \\ \cline{2-3}
         & Thurst-to-weight Ratio &  9.74  \\
         & Mass & 0.55 [\SI{}{\kilogram}] \\
         & Maximum Thrust & 13.14 $\times$ 4 [\SI{}{\newton}] \\
         & Arm Length & 0.15 [\SI{}{\meter}] \\
         & Inertia (x-axis) & 0.001369 [\SI{}{\kilogram\square\meter}] \\
         & Inertia (y-axis) & 0.001338 [\SI{}{\kilogram\square\meter}] \\
         & Inertia (z-axis) & 0.002452 [\SI{}{\kilogram\square\meter}] \\
         & Motor Time Constant & 0.02 [\SI{}{\second}] \\
         & System Delay &  0.03 [\SI{}{\second}] \\
        \bottomrule
    \end{tabular}
\end{table}


==> Images/objectives_tikz_mpc_rl.tex <==
\begin{figure}[!htp]
\centering
\begin{tikzpicture}
\begin{scope}%[xshift=1.5cm]
    \fontsize{9.5pt}{12pt}\selectfont
    % 
    \node [mybox] (box) at (1,0) {%
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=1\textwidth]{Images/obj_tracking.png} 
        \end{minipage}
    };
    \node[fancytitle, right=10pt] at (box.north west) {Trajectory Tracking};
    % 
    \node [mybox] (box) at (9,0) {%
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=1\textwidth]{Images/obj_progress.png}
        \end{minipage}
    };
    \node[fancytitle, right=10pt] at (box.north west) {Progress Maximization};
\end{scope}
\begin{scope}[yshift=-1.5cm]
\node [anchor=west] (note) at (3, 2.7) {\color{black} G2};
    \node [anchor=west] (note) at (1, 1.0) {\color{black} $s_t, \cdots, s_{t+N}$};
    \node [anchor=west] (note) at (1, 2.2) {\color{black} $r_t, \cdots, r_{t+N}$};
    % 
    \node [anchor=west] (note) at (11, 2.7) {\color{black} G2};
    \node [anchor=west] (note) at (9, 1) {\color{black} $s_t, \cdots, s_{t+N}$};
\end{scope}

\end{tikzpicture}%
\\
% \includegraphics[width=1\linewidth]{Images/comparison.png}
% \includegraphics[width=1\linewidth]{Images/comparison_xy.png}
% \includegraphics[width=1\linewidth]{Images/comparison_yz.png}
% \includegraphics[width=1\textwidth]{Images/rl_sparrow_arrow.pdf};
\caption{An illustration of trajectory tracking and progress maximization. } 
\label{fig:mpc_rl_objectives}
\end{figure}

==> Images/optimization_tikz.tex <==
\begin{figure}[htp]
\centering
\begin{tikzpicture}

\begin{scope}%[xshift=1.5cm]
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=1\textwidth]{Images/optimization.pdf}};
\end{scope}
\begingroup
    \fontsize{9pt}{12pt}\selectfont
    \node [anchor=west] (note) at (0.8, 1.5) {$\nabla J$};
    \node [anchor=west] (water) at (5.3, 1.5) { $\nabla J$};
    % 
    \node [anchor=west] (note) at (1.5, 4.0) {\color{black} The Choice of Optimization Method};
    \node [anchor=west] (note) at (10, 4.0) {\color{black} The Choice of Optimization Objective};
\endgroup
\end{tikzpicture}%
\caption{
A taxonomy of our \textit{Optimization Method versus Optimization Objective} hypothesis. 
} 
\label{fig: hypothesis}
\end{figure}


==> Images/timelapse_drones.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{Images/drone_stack.png}
\caption{
\textbf{Time-lapse illustrations of a high-performance racing drone controlled by our RL policy.}
% 
We test on two race tracks, the Split-S track \textbf{(A)} and the Marv track \textbf{(B)}; both are designed by world-class human drone pilots.   
% 
Our RL policy achieves a peak speed of \SI{108}{\kilo\meter\per\hour} and a peak acceleration greater than \SI{12}{\g} in an indoor flying arena.
Recordings of the experiments can be found in Movie~1.
} 
\label{fig: overview}
\end{figure*}

==> Sections/abstract.tex <==
\begin{sciabstract}
A central question in robotics is how to design a control system for an agile mobile robot.
% 
This paper studies this question systematically, focusing on a challenging setting: autonomous drone racing. 
%
We show that a neural network controller trained with reinforcement learning (RL) outperforms optimal control (OC) methods in this setting.
% 
We then investigate which fundamental factors have contributed to the success of RL or have limited OC. 
% 
% Our study indicates that the fundamental advantage of RL over OC lies in its optimization objective.
Our study indicates that the fundamental advantage of RL over OC is not that it
optimizes its objective better but that it optimizes a better objective.
% 
OC decomposes the problem into planning and control with an explicit intermediate representation, \final{such as a trajectory}, that serves as an interface.
% 
This decomposition limits the range of behaviors that can be expressed by the \rebuttal{controller}, leading to inferior control performance when facing unmodeled effects.
% 
\rebuttal{In contrast, RL can directly optimize a task-level objective and can leverage domain randomization to cope with model uncertainty, allowing the discovery of more robust control responses.}
% 
% Within minutes of training on a standard workstation, our policy achieves superhuman control and pushes an agile racing drone to its physical limit, achieving a peak acceleration greater than 117 meters per second squared and a peak velocity of 108 kilometers per hour. 
% 
Our findings allow us to push an agile drone to its maximum performance, achieving a peak acceleration greater than \final{12 times the gravitational acceleration and a peak velocity of 108 kilometers per hour}. Our policy achieves superhuman control within minutes of training on a standard workstation. 
% 
This work presents a milestone in agile robotics and sheds light on the role of RL and OC in robot control.
\end{sciabstract}


==> Tables/hypotheses.tex <==
\begin{table}[!htp]
    % \small
    \centering
    \fontsize{8pt}{12pt}\selectfont   
    \caption{A taxonomy of the \textit{Reinforcement-Learning-Surpass-Optimal-Control} hypothesis. }
    \label{tab:results_overview}
    \begin{tabular}{ @{}l | c | c }
        \toprule
        x
        & Reinforcement Learning
        & Optimal Control   \\
        \hline
        x & x & x \\
        \bottomrule
        \multicolumn{3}{c}{\includegraphics[width=1\linewidth]{Images/optimization.pdf}}
    \end{tabular}
\end{table}



==> timelapse_drones.tex <==
\begin{figure}[!htp]
\centering
\includegraphics[width=1\textwidth]{Images/drone_stack.png}
%\includegraphics[width=1\textwidth]{Images/drone_stack_marv_low.png}
\caption{
\textbf{Time-lapse illustrations of a high-performance racing drone controlled by our RL policy.}
% 
We test on two race tracks, the Split-S track \textbf{(A)} and the Marv track \textbf{(B)}; both are designed by world-class human drone pilots.   
% 
Our RL policy achieves a peak speed of \SI{108}{\kilo\meter\per\hour} and a peak acceleration greater than \SI{12}{\g} in an indoor flying arena.
} 
\label{fig: overview}
\end{figure}
